Sensor-based Proximity Detection in the Face of Active Adversaries

Contextual proximity detection (or, co-presence detection) is a promising approach to defend against relay attacks in many mobile authentication systems. We present a systematic assessment of co-presence detection in the presence of a context-manipulating attacker. First, we show that it is feasible to manipulate, consistently control and stabilize the readings of different acoustic and physical environment sensors (and even multiple sensors simultaneously) using low-cost, off-the-shelf equipment. Second, based on these capabilities, we show that an attacker who can manipulate the context gains a significant advantage in defeating context-based co-presence detection. For systems that use multiple sensors, we investigate two sensor fusion approaches based on machine learning techniques: features-fusion and decisions-fusion, and show that both are vulnerable to contextual attacks but the latter approach can be more resistant in some cases.

==> relatedwork.tex <==
There has been an extensive research on defending against relay attacks. The traditional
defense, distance bounding \cite{brands1993distance,Hancke05,Reid07},
requires high accuracy in measuring round trip time of messages between \prover
and \verifier. This solution may therefore be difficult to implement in practice. The
limitation of distance bounding has been mentioned in various existing works, such
as \cite{DBLP:conf/esorics/HaleviMSX12}, \cite{ShresthaFC2014}.    

%One of the approaches to prevent against a relay attack is to use Distance
%Bounding techniques \cite{brands1993distance}. \cite{Hancke05, Reid07} has worked on to
%detect and prevent relay attack using timing-based protocols. However, such
%prevention using the time for signal propagation is highly sensitive to the
%delays in the system. These systems needs dedicated hardware which should have
%no delays as a delay of one nano second might result into an error of 30
%centimeters. 

As discussed before, the other way to thwart relay attacks is to use the context of the 
location (contextual proximity detection).  There has been extensive research  
 to prevent relay attacks using different kinds of context. 
% A context of
%a location is any information that can be used to identify a location and
%differentiate it from other locations. 
\begin{comment}
These contexts can either be natural or artificial. 
The ambient information such as audio, radio (\wifi, \bluetooth,
{\bf GPS}) and physical environment such as \temperature, \altitude, \humidity, \gas
and other natural information that can be used to identify a location where
a device is.

\end{comment}
%
%
%Similarly, RFID signals such as \wifi, \bluetooth or GPS signals etc are
%artificial information which can be used to identify a location. Many
%researchers have selected either one of these or combinations of these to
%provide a contextual information such that relay attack can be thwarted.
%
%audio
To detect co-presence using ambient audio, Halevi et al.
\cite{DBLP:conf/esorics/HaleviMSX12} analyzed different methods such as
time-based, frequency-based and time-frequency based similarity detection using
raw audio data. Besides preventing relay attacks, ambient audio has been used for securing communications such
as in \cite{nguyen2012using,schurmann2013audio}.  Nguyen et al.
\cite{nguyen2012using} used pattern based audio alignment for secure
communication between mobile phones using ambient audio
\cite{nguyen2012pattern}. Similarly Schurmann et al.  \cite{schurmann2013audio}
tried to establish a secure communication channel among devices based on
similar audio patterns.
%
%Wi-Fi + \bluetooth
Prior work on co-presence detection also used RF
signals such as Wi-Fi and Bluetooth \cite{douse2012place,krumm2004nearme,Mathur11proximate,Narayanan11,varshavsky07amigo}. 
In \cite{douse2012place},
Dousse et al. used the list of available Wi-Fi APs to learn the place.
Narayanan et al. in \cite{Narayanan11} discussed how to create a location tags
using various RF and physical sensors. They suggested to create location tags
using Wi-Fi access points and broadcast packets. They also suggested the use of GPS, GSM, audio, or gases to
generate the location tags, which they deferred to future work. Krumm et al. used
Wi-Fi similarity features for proximity detection in \cite{krumm2004nearme}.
BlueProximity app in sourceforge \cite{BlueProximity} uses bluetooth to
authenticate devices.

\begin{comment}
%GPS
Ma et al. in \cite{Ma13} used GPS for enhancing security and privacy in
RFID cards with GPS sensing capabilities. They suggest that location awareness
by location or location related information (such as speed) can serve as
a legitimate access context. They used external GPS modules to provide context
comparison enhancing simple RFID authentication. In their approach, they
attempt to authorize the device by detecting the proximity between the sensed
location and the preset legitimate locations. The device is authorized only if
its location vector falls into a square region centered at a legitimate
location.  According to the experiment result of the location-based selective
authorization, location information acquired from GPS is strong and accurate
context information for detecting co-presence.
\end{comment}

%our paper - fusion of sensor modalities
As discussed earlier, Shrestha et al. \cite{ShresthaFC2014} explored the use of four purely ambient
physical modalities (temperature, humidity, altitude and gas) for co-presence detection. They provided accuracy of
individual modalities as well as combination of modalities. According to their
analysis, \altitude provided the best accuracy to make the decision while they
suggest that combining multiple sensor modalities provides better accuracy to
detect the co-presence.  Truong et al. 
\cite{TruongPerCom14} compared different audio and radio sensor modalities to
detect co-presence.  They also provided detailed comparison of each modality
versus (feature level) fusion of modalities. 
They only reported the performance of single modality unidirectional
attack. According to their analysis, Wi-Fi provided near perfect results and
is the most effective sensor modality for co-presence detection.


